Universal Domain Adaptation in Ordinal Regression

We address the problem of universal domain adaptation (UDA) in ordinal regression (OR), which attempts to solve classification problems in which labels are not independent, but follow a natural order. We show that the UDA techniques developed for classification and based on the clustering assumption, under-perform in OR settings. We propose a method that complements the OR classifier with an auxiliary task of order learning, which plays the double role of discriminating between common and private instances, and expanding class labels to the private target images via ranking. Combined with adversarial domain discrimination, our model is able to address the closed set, partial and open set configurations. We evaluate our method on three face age estimation datasets, and show that it outperforms the baseline methods.

==> 5-table_cacd.tex <==
%-----------------------------------------
\begin{footnotesize}
\begin{table*}[!ht]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} \hline 
Task &\multicolumn{2}{c|}{AFAD$\ra$CACD} 
       &\multicolumn{2}{c|}{CACD$\ra$AFAD}
         &\multicolumn{2}{c|}{AFAD$\ra$CACD}
           &\multicolumn{2}{c|}{CACD$\ra$AFAD}       \\ 
     &\multicolumn{2}{c|}{[15-40]$\ra$[15-62]} 
       &\multicolumn{2}{c|}{[15-62]$\ra$[15-40]}
         &\multicolumn{2}{c|}{[15-40]$\ra$[15-40]}
           &\multicolumn{2}{c|}{[15-40]$\ra$[15-40]} \\ \hline
Configuration &\multicolumn{2}{c|}{OS ($\xi=0.53$)}
        &\multicolumn{2}{c|}{PA ($\xi=0.53$)} 
          &\multicolumn{2}{c|}{SC ($\xi=1.0$)} 
            &\multicolumn{2}{c|}{SC ($\xi=1.0$)}     \\ \hline
No adaptation & 3.37&15.82 & 6.55&18.89  & 3.37&8.72  & 4.40&7.42  \\
ORUDA         & 3.34&12.43 & 5.83&10.31  & 3.34&7.16 &  4.38&6.19    \\ 
Supervised    & 3.37&6.55  & 6.55&3.37   & 3.37&6.55  & 4.40&3.37  \\ 
\hline
Task &\multicolumn{2}{c|}{CACD$\ra$UTKFace} 
       &\multicolumn{2}{c|}{CACD$\ra$UTKFace}
         &\multicolumn{2}{c|}{UTKFace$\ra$CACD}
           &\multicolumn{2}{c|}{CACD$\ra$UTKFace}     \\ 
     &\multicolumn{2}{c|}{[15-62]$\ra$[1-50]} 
       &\multicolumn{2}{c|}{[15-62]$\ra$[30-80]}
         &\multicolumn{2}{c|}{[15-62]$\ra$[1-80]}
           &\multicolumn{2}{c|}{[1-80]$\ra$[15-62]} \\ \hline
Configuration &\multicolumn{2}{c|}{OSPA ($\xi=0.38$)}
        &\multicolumn{2}{c|}{OS ($\xi=0.40$)} 
          &\multicolumn{2}{c|}{PA ($\xi=0.40$)} 
            &\multicolumn{2}{c|}{SC ($\xi=1.0$)}      \\ \hline
No adaptation & 5.86&9.87 &  5.86&10.79 & 5.86&19.53 & 3.39&13.32 \\
ORUDA         & 5.88&7.88 &  5.91&8.50  & 5.94&11.12 & 3.38&9.75  \\ 
Supervised    & 5.86&5.33 &  5.86&6.72  & 5.86&5.20  & 3.39&4.33  \\ 
\hline
\end{tabular}
\label{tab:cacd}
\caption{Evaluation for the domain pairs: AFAD-CACD and UTKFace-CACD. The values reported are MAE (source) and e-MAE (target).}
\end{center}
\end{table*}
\end{footnotesize}



==> 5-table_cacd_baselines.tex <==
%-----------------------------------------
\begin{footnotesize}
\begin{table}[!ht]
\scriptsize
\begin{center}
\setlength\tabcolsep{5pt}
\begin{tabular}{|c|c|c|c|c|c|} \hline 
Source&A[15-40] &C[15-40]&C[15-62]&\multicolumn{2}{c|}{A[15-40]} \\ \hline
Target&C[15-40] &A[15-40]&A[15-40]&\multicolumn{2}{c|}{C[15-62]} \\ \hline
Config($\xi$) &CS(1.0) &CS(1.0) &PA(0.53)&\multicolumn{2}{c|}{OS(0.53)} \\ \hline
Setup &   MAE &   MAE  & MAE  &  MAE&e-MAE \\ \hline
No adaptation 
      &  8.72 &  7.42  & 17.95 & 15.67  & 15.82   \\
PADA~\cite{cao2018-eccv}  
      &  7.71 &  7.11  & 15.71   &  -   & -      \\
OPDA-BP~\cite{Saito_2018_ECCV}  
      &  7.48 &  6.84  &  -      & 14.51& -    \\
UAN~\cite{you2019universal}  
      &  7.57 &  6.73  & 15.75   & 14.79& -      \\
DANCE~\cite{saito20universal} 
      &{\bf 7.13}&6.43- & 15.23  & 14.17 & -    \\
ORUDA(ours)  
      & 7.26 &{\bf 6.19}&{\bf 10.31}&{\bf 12.48}&{\bf 12.43} \\ \hline
Supervised  
      & 6.55  & 3.37   &  6.52   &6.49 &6.41     \\ 
\hline
\end{tabular}
\label{tab:afad-cacd}
\caption{Evaluation for AFAD(A)-CACD(C) pair.
The table reports MAE values for CS, PA and OS tasks and e-MAE values for OS case.}
\end{center}
\end{table}
\end{footnotesize}

%----------------------------------------------------
\begin{footnotesize}
\begin{table}[!ht]
\scriptsize
\begin{center}
\setlength\tabcolsep{4.5pt}
\begin{tabular}{|c|c|c|cc|cc|} \hline 
Source &C[1-80] &U[15-62]&\multicolumn{2}{c|}{C[15-62]}
              &\multicolumn{2}{c|}{C[15-62]}  \\ \hline
Target &U[15-62]&C[1-80] &\multicolumn{2}{c|}{U[30-80]}
              &\multicolumn{2}{c|}{U[1-50]}   \\ \hline
Config($\xi$) &CS(1.0) &PA(0.40) &\multicolumn{2}{c|}{OS(0.40)} 
                    &\multicolumn{2}{c|}{OSPA(0.38} \\  \hline
Setup &MAE &MAE &MAE &e-MAE &MAE &e-MAE \\ \hline
No adaptation& 13.32  & 19.53  & 10.79&10.79 & 9.87&9.87  \\
PADA~\cite{cao2018-eccv} 
             & 10.71  & 14.60  &     - & -   &  -  & -     \\
OPDA-BP~\cite{Saito_2018_ECCV} 
             & 10.68  & -      & 10.33 & -   &  -  & -      \\
UAN~\cite{you2019universal} 
             & 10.67  & 14.74  & 10.39 & -   & 9.75& -      \\
DANCE~\cite{saito20universal}
             &10.33   & 14.53  &  9.87 & -   & 9.43& -     \\
ORUDA(ours)  &{\bf 9.75}&{\bf 11.12}&{\bf 8.91}&{\bf 8.50}&{\bf 7.79}&{\bf 7.88} \\ \hline
Supervised   & 4.33   & 5.20   &  6.86 &6.72 & 5.86&5.33  \\ 
\hline
\end{tabular}
\label{tab:utk-cacd}
\caption{Evaluation for UTKFace(U)-CACD(C) pair. The table reports MAE values for CS, PA, OS and OSPA tasks and e-MAE values for OS and OSPA cases. %'A' stands for ACAD, 'C' stands for CACD.
}
\end{center}
\end{table}
\end{footnotesize}



==> 5-table_utk_afad.tex <==
%-----------------------------------------
\begin{footnotesize}
\begin{table*}[!ht]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} \hline 
Task &\multicolumn{2}{c|}{AFAD$\ra$UTKFace} 
         &\multicolumn{2}{c|}{AFAD$\ra$UTKFace}
             &\multicolumn{2}{c|}{UTKFace$\ra$AFAD}
                 &\multicolumn{2}{c|}{AFAD$\ra$UTKFace} \\
     &\multicolumn{2}{c|}{[15-40]$\ra$[1-30]} 
         &\multicolumn{2}{c|}{[15-40]$\ra$[1-80]}
             &\multicolumn{2}{c|}{[1-80]$\ra$[15-40]}
                 &\multicolumn{2}{c|}{[15-40]$\ra$[15-40]} \\ \hline
Configuration &\multicolumn{2}{c|}{OSPA ($\xi=0.38$)}
         &\multicolumn{2}{c|}{OS ($\xi=0.15$)} 
             &\multicolumn{2}{c|}{PA ($\xi=0.31$)} 
                 &\multicolumn{2}{c|}{SC ($\xi=1.0$)} \\ \hline
No adaptation & 3.39&9.87 & 3.37&11.62 & 5.20&8.44 & 3.37&5.01 \\
UDA~\cite{you2019universal} 
              & 3.38&9.75 & 3.35&11.51 & 5.22&8.34 & 3.38&4.74 \\
ORUDA         & 3.38&7.70 & 3.23&9.55  & 4.88&5.39 & 3.38&4.70 \\ 
Supervised    & 3.40&4.91 & 3.37&5.30  & 5.20&3.39 & 3.37&4.37 \\ 
\hline
\end{tabular}
\label{tab:utk_afad}
\caption{The evaluation results for UTKFace-AFAD domains. The values reported are MAE (source) and e-MAE (target).}
\end{center}
\end{table*}
\end{footnotesize}


==> 5-table_utk_afad_baselines.tex <==
%-----------------------------------------
\begin{footnotesize}
%\begin{table*}[!hb]
\begin{table}[!ht]
%\tiny
\scriptsize
\begin{center}
\setlength\tabcolsep{4.5pt}
\begin{tabular}{|c|c|c|cc|cc|} \hline 
%UDA Task 
%    &A[15-40]$\rightarrow$U[15-40] 
%        &A[1-80]$\rightarrow$U[15-40]
%           &\multicolumn{2}{c|}{A[15-40]$\rightarrow$u[1-80]}
%              &\multicolumn{2}{c|}{A[15-40]$\rightarrow$U[1-30]} 
%                 \\ \hline
%Configuration  
%    &CS($\xi=1.0$) 
%        &PA($\xi=0.31$) 
%            &\multicolumn{2}{c|}{OS ($\xi=0.15$)} 
%               &\multicolumn{2}{c|}{OSPA ($\xi=0.38$)}
%                  \\ \hline
Source &A[15-40]&A[1-80] &\multicolumn{2}{c|}{A[15-40]}
                                &\multicolumn{2}{c|}{A[15-40]} \\ \hline
Target &U[15-40]&U[15-40]&\multicolumn{2}{c|}{U[1-80]}
                                &\multicolumn{2}{c|}{U[1-30]}  \\ \hline
Config($\xi$) &CS(1.0)&PA(0.31)&\multicolumn{2}{c|}{OS(0.15)}&\multicolumn{2}{c|}{OSPA(0.38)}\\ \hline

Setup &MAE &MAE &MAE &e-MAE &MAE &e-MAE \\ \hline
%Setup &Mae &Mae &Mae &eMae &Mae &eMae \\ \hline

No adaptation & 5.01 & 8.44 & 11.43& 11.62 & 9.76&9.87  \\ 
PADA~\cite{cao2018-eccv} 
              & 4.72& 7.71 &  -   &-   & -    & -      \\
OPDA-BP~\cite{Saito_2018_ECCV} 
              & 4.68 & - & 11.51& - & -   &-             \\
UAN~\cite{you2019universal} 
              & 4.74 & 7.67 & 11.39& - & 9.75&-         \\
%UAN~\cite{you2019universal} + Coral
%              & {\bf 4.53} & 7.36 & 11.23& - & 9.57&-         \\
DANCE~\cite{saito20universal}
              & {\bf 4.53} & 7.36 & 11.23& - & 9.57&-         \\
ORUDA(ours)   & 4.70 & {\bf 5.39} & {\bf 9.36}&{\bf 9.55} &{\bf 7.81}&{\bf 7.70}  \\ \hline
Supervised    & 4.37 & 3.39 & 5.37&5.30 & 4.84&4.91   \\ 
\hline
\end{tabular}
\label{tab:utk_afad}
\caption{Evaluation for UTKFace(U)-AFAD(A) pair. The table reports MAE values for CS, PA, OS and OSPA tasks and e-MAE values for OS and OSPA cases.}
\end{center}
\end{table}
\end{footnotesize}


==> weighted-eMAE.tex <==
%-----------------------------------------
\begin{footnotesize}
%\begin{table*}[!hb]
\begin{table*}[!ht]
%\tiny
\scriptsize
\begin{center}
\setlength\tabcolsep{2.2pt}
\begin{tabular}{|c||c|c|cc|cc||c|c|cc|cc||c|c|c|cc|} \hline 
Domain pairs
&\multicolumn{6}{c||}{AFAD(A) - UTKFace(U)} &\multicolumn{6}{c||}{CACD(C) - UTKFace(U)}
&\multicolumn{5}{c|}{CACD(C) - AFAD(A)}
\\ \hline
Source 
&A[15-40]&A[1-80] &\multicolumn{2}{c|}{A[15-40]}&\multicolumn{2}{c||}{A[15-40]} 
&C[1-80] &U[15-62]&\multicolumn{2}{c|}{C[15-62]} &\multicolumn{2}{c||}{C[15-62]}
&A[15-40] &C[15-40]&C[15-62]&\multicolumn{2}{c|}{A[15-40]}
\\ \hline
Target 
&U[15-40]&U[15-40]&\multicolumn{2}{c|}{U[1-80]}  &\multicolumn{2}{c||}{U[1-30]} 
&U[15-62]&C[1-80] &\multicolumn{2}{c|}{U[30-80]} &\multicolumn{2}{c||}{U[1-50]} 
&C[15-40] &A[15-40]&A[15-40]&\multicolumn{2}{c|}{C[15-62]}
\\ \hline
Config($\xi$) 
&CS(1.0) &PA(0.31) &\multicolumn{2}{c|}{OS(0.15)}&\multicolumn{2}{c||}{OSPA(0.38)}
&CS(1.0) &PA(0.40) &\multicolumn{2}{c|}{OS(0.40)} &\multicolumn{2}{c||}{OSPA(0.38}
&CS(1.0) &CS(1.0)  &PA(0.53)&\multicolumn{2}{c|}{OS(0.53)}
\\ \hline
Setup 
&e-MAE &we-MAE &e-MAE &we-MAE &e-MAE &we-MAE 
&e-MAE &we-MAE &e-MAE &we-MAE
\\ \hline \hline
No adaptation 
& 11.43 & 11.62 
& 9.76  & 9.87  
& 10.79 & 10.79 
& 9.87  & 9.87 
& 15.67 & 15.82
\\ \hline



ORUDA(ours)   
& 4.70 & {\bf 5.39} & {\bf 9.36}&{\bf 9.65} &{\bf 7.81}&{\bf 7.70}
&{\bf 9.75}&{\bf 11.12}&{\bf 8.91}&{\bf 8.95}&{\bf 7.79}&{\bf 7.88}
& 7.26 &{\bf 6.19}&{\bf 10.31}&{\bf 12.48}&{\bf 12.57}
\\ \hline

\hline
\end{tabular}
\caption{Evaluation of 12 UDA tasks defined on AFAD-UTKFace, CACD-UTKFace and CACD-AFAD domain pairs. MAE values are reported for CS, PA, OS and OSPA tasks; e-MAE values are reported for OS and OSPA tasks.}
\label{tab:eval}
\end{center}
\end{table*}
\end{footnotesize}

